On the Challenges of Cosmic-Ray Proton Shock Acceleration in the Intracluster Medium

Galaxy clusters host the largest particle accelerators in the Universe: Shock waves in the intracluster medium (ICM), a hot and ionised plasma, that accelerate particles to high energies. Radio observations pick up synchrotron emission in the ICM, proving the existence of accelerated cosmic-ray electrons. However, a sign of cosmic-ray protons, in form of $\gamma$-rays. remains undetected. This is know as the missing $\gamma$-ray problem and it directly challenges the shock acceleration mechanism at work in the ICM. Over the last decade, theoretical and numerical studies focused on improving our knowledge on the microphysics that govern the shock acceleration process in the ICM. These new models are able to predict a $\gamma$-ray signal, produced by shock accelerated cosmic-ray protons, below the detection limits set modern $\gamma$-ray observatories. In this review, we summarise the latest advances in solving the missing $\gamma$-ray problem.

==> cite.tex <==
citep[e.g.][]{2015SSRv..188...93P}. These highly energetic processes drive both shock waves and turbulence in the ICM, giving rise to large acceleration sites for cosmic-rays. Radio observations of diffuse synchrotron emission proof the acceleration of cosmic-ray electrons in the ICM as well as the existence of large-scale magnetic fields \citep[e.g.][]{2008SSRv..134...93F,2012A&ARv..20...54F,vanweeren2019review}. Following the definition by \citep{vanweeren2019review}, diffuse radio sources in the ICM are classified into three groups: 1) giant radio halos and mini-haloes, 2) radio relics (or radio shocks) and 3) revived AGN fossil plasma sources. While the origin of the latter sources is still debated, it is commonly assumed that halos and relics are produced by cosmic-ray electrons that have been (re-)accelerated by ICM turbulence and shocks, respectively. On the other hand, any signatures of cosmic-ray protons in the ICM are still waiting for their detection. In the case of radio halos, the non-detection of cosmic-ray protons favors the turbulent re-acceleration model \citep[e.g.][and references therein]{2001MNRAS.320..365B,2001ApJ...557..560P,donn10,2013MNRAS.429.3564D,2014MNRAS.443.3564D,2017MNRAS.465.4800P} over the hadronic (or secondary) models \citep[e.g.][and references therein]{1980ApJ...239L..93D,1999APh....12..169B,2008MNRAS.385.1211P,2011A&A...527A..99E} for the origin of radio haloes \citep[e.g.][]{2011ApJ...728...53J,2017MNRAS.472.1506B}. On the other hand, in the case of radio relics, the non-detection of cosmic-ray protons directly challenges the shock acceleration mechanisms in the ICM \citep[e.g.][]{va14relics}
cite{wittor2020gammas}: expected $\gamma$-ray emission (color) of two clusters from the simulated sample. The white contours give the baryonic density and the red circle marks the $r_{200}$. }
citep[e.g.][]{2013MNRAS.433.1701O,2013PASJ...65...16A,2016MNRAS.460L..84B,2016MNRAS.463.1534B,2018MNRAS.478.2218H} gave rise to the idea that ICM electrons are shock accelerated to high energies, where they emit synchrotron radiation \citep{ensslin1998}. The originally proposed acceleration mechanism is diffusive shock acceleration \citep[DSA, see][for physical details]{1978ApJ...221L..29B,1978MNRAS.182..147B,1978MNRAS.182..443B,1983RPPh...46..973D,1987PhR...154....1B,2014IJMPD..2330007B,bykov2019review,marcowith2020review}. While this picture is commonly accepted, some open questions remain. In several cases, the Mach number estimates from X-ray and radio observations yield different shock strengths \citep[][]{2014MNRAS.445.1213S,2015ApJ...812...49H,2016ApJ...818..204V,Hoang2017sausage}. In addition, while the radio power of some relics is explained by the shock acceleration from the thermal pool  \citep{locatelli2020dsa}, several other relics require shock re-acceleration \citep[e.g.][]{2014ApJ...785....1B,2017NatAs...1E...5V,Stuardi2019}. In this review, we concentrate on the \textit{missing $\gamma$-ray problem}
citep{1999APh....12..169B}
citep{1980ApJ...239L..93D}.}, (see Fig. \ref{fig::maps}). However, such signal has not been detected so far \citep[e.g.][]{ackermann14,ackermann15,ackermann16,Huber2013}. This non-detection poses a fundamental challenge on the shock acceleration mechanisms in the ICM. Several solutions have been proposed to explain the non-detection of $\gamma$-rays: modifying the cosmic-ray proton distribution in clusters \citep[e.g.][]{2011A&A...527A..99E,2013MNRAS.434.2209W,2014MNRAS.438..124Z,2017MNRAS.465.4800P}, revising the particle acceleration efficiencies \citep[e.g.][]{va14relics,2015MNRAS.451.2198V,ka12,2013MNRAS.435.1061P} and a better understanding of the microphysical processes of the shock acceleration mechanism \citep[e.g.][]{2014ApJ...783...91C,2014ApJ...794...46C,2014ApJ...794...47C,Guo_eta_al_2014_I,Guo_eta_al_2014_II,Ha2018protons,Ryu2019,2017JKAS...50...93K,2018ApJ...856...33K,2020JKAS...53...59K}
citep[e.g.][]{ackermann14,2014ApJ...795L..21G,zand14,aha09,alek10,alek12,alek14,ahnen16}. While ground-based observations mostly probe the energy range above $\gtrsim 1  \ \GeV$, space-based observations are mostly looking at energies between $\sim 100 \ \MeV $ and $\sim 1 \ \TeV$. Theoretical estimates yield that the $\gamma$-ray emission in the ICM is expected to be the strongest around $\sim 1 \ \GeV$ \citep{2017MNRAS.472.1506B,2010MNRAS.409..449P}, hence, favoring space-based observations to detect $\gamma$-rays. Though, ground- and space-based observations do not compete but very well complement each other \citep[e.g.][]{arl12}. However, none of them has ever reported the detection of a $\gamma$-ray signal from the ICM. Hence, they all provide upper limits on the $\gamma$-ray flux expected from cosmic-ray protons in the ICM. The deepest upper limits have been set by the Large Area Telescope\footnote{http://www-glast.stanford.edu/} on board of the Fermi Satellite\footnote{https://fermi.gsfc.nasa.gov/}
citep[e.g.][for technical details]{2009ApJ...697.1071A,ack12tech} and, hence, it perfectly covers the desired energy range around $\sim 1 \ \GeV$ \citep[e.g.][]{2017MNRAS.472.1506B,2010MNRAS.409..449P}. Using Fermi-LAT's 4 year all-sky data, \cite{ackermann14} searched for spatially extended $\gamma$-ray emission in a sample of 50 X-ray bright galaxy clusters that included both cool-core and non-cool-core clusters. Using the cosmic-ray model by \cite{2010MNRAS.409..449P}, they thoroughly analysed the sample. Yet, they did not report any $\gamma$-ray emission attributed to the ICM. Hence, they presented upper limits for the $\gamma$-ray flux above $500 \ \MeV$ that are between $0.5$ and $22.2 \cdot 10^{-10} \ \mathrm{ph \ cm^{-2} \ s^{-1}}
citep{ackermann15} and the Coma cluster \citep{ackermann16}. Albeit, these observations used a larger energy range, i.e. $\ge 100 \ \MeV$, and, in the case of Coma, 6 years of data, they did not report any $\gamma$-ray signal. Hence, the $\gamma$-ray flux limits are $5.2 \cdot 10^{-9} \ \mathrm{ph \ cm^{-2} \ s^{-1}}$ and $1.2 \cdot 10^{-8} \ \mathrm{ph \ cm^{-2} \ s^{-1}}$ for Coma and Virgo, respectively. In an independent work, \cite{zand14} used 63 months of Fermi-LAT observations to analyse the Coma cluster in the energy $100 \ \MeV$ to $100 \ \GeV$. For different physical scenarios, they found upper limits in the range of $10^{-10}$ to $10^{-9} \ \mathrm{ph \ cm^{-2} \ s^{-1}}
cite{2013AA...560A..64H} used the stacking of $\gamma$-ray counts maps \citep[also see][]{2012A&A...547A.102H} to estimate statistical upper limits on a sample of 53 galaxy clusters taken from the HIFLUGS catalog \citep{Reiprich:2002}. For energies between $1$ and $300 \ \GeV$, they found an upper limit of a few $10^{-11} \ \mathrm{ph \ cm^{-2} \ s^{-1}}$ for their whole sample . Furthermore, they performed separate stacking analyses for cool-core and non-cool-core clusters, that yielded upper limits of $5.7$ and $2.7 \cdot 10^{-11} \mathrm{ph \ cm^{-2} \ s^{-1}}$, respectively. \cite{2014ApJ...795L..21G} performed an independent stacking analysis using 78 nearby clusters. In the $0.8$ to $100 \ \GeV$ energy band, they recorded an upper limit of $2.3 \cdot 10^{-11} \ \mathrm{ph \ cm^{-2} \ s^{-1}}
citep{2016MNRAS.459...70V}
citep[e.g.][]{ryu2003}
cite{2016MNRAS.459...70V} tested a variety of acceleration efficiencies (that we discuss further below). They found that the efficiencies, available at that time, were too large and produced visible $\gamma$-rays. Furthermore, they showed that an overall constant acceleration efficiency of $\eta = 10^{-3}$ would be required to make galaxy clusters undetectable to current instruments. A word of caution: simply lowering the acceleration efficiencies is difficult to be brought in line with the observations of radio relics. Especially as low acceleration efficiencies already have difficulties in explaining the radio power of several observed relics \citep[e.g.][]{2014ApJ...785....1B,2017NatAs...1E...5V,Stuardi2019}
cite{Ryu2019}: cosmic-ray acceleration efficiencies as a function of Mach number. The red and black lines give the efficiencies for injection moments of $p_{\mathrm{inj}} = 3.5 \cdot p_{\mathrm{th}}$ (red) and $p_{\mathrm{inj}} = 3.3 \cdot p_{\mathrm{th}}$ (red), where $p_{\mathrm{th}}$ is the momentum of the thermal post-shock electrons. The circles show the results, if the injection momentum is assumed as a lower bound for computing the injection fraction, while the triangles assume the threshold energy for the pion-production reaction, $780 \ \MeV/c$, as a lower bound. The points at $M_\mathrm{s} = 2$ and $M_{s} = 1.5$ are not able to accelerate protons. However, they are plotted for completeness.}
cite{kj07} used 1D diffusion convection equations of shocks to estimate the shock acceleration efficiencies. Using a similar model, \cite{2007A&A...473...41E} derived acceleration efficiencies for different post-shock temperatures. However, both of these are above the $\eta = 10^{-3}$ limit given by \cite{2016MNRAS.459...70V}. By including more microphysical effects, \cite{2013ApJ...764...95K,2014ApJ...783...91C,Ryu2019} updated the efficiencies given in \cite{kj07}, always yielding lower efficiencies. \cite{2013ApJ...764...95K} included energy dissipation due to Alfven waves that are amplified at the shock. \cite{2014ApJ...783...91C} took into account the effect of the shock obliquity on the acceleration process (see discussion below), which gives efficiencies that are half the efficiencies derived by \cite{2013ApJ...764...95K}. Finally, \cite{Ryu2019} also included the dynamical feedback of cosmic-ray pressure on the shock. This model yields acceleration efficiencies, see Fig. \ref{fig::ryu2019}, that are lower than the ones of its predecessors and that fall below the $\eta = 10^{-3}$ limit given by \cite{2016MNRAS.459...70V}. Yet, it was shown that these efficiency reduce the $\gamma$-ray emission significantly, but not enough to make galaxy clusters invisible in $\gamma$-rays \citep[e.g.][and below]{wittor2020gammas}
citep{2014ApJ...783...91C,Ha2018protons}. Shocks can be characterized by two properties: their strength, given by the Mach number, and their orientation to the underlying magnetic field, given by the shock obliquity. The latter is defined as the angle between shock normal, $\mathbf{n_{shock}}$, and magnetic field, $\mathbf{B}
cite{Ha2018protons}
cite{2014ApJ...783...91C} found that cosmic-ray protons require quasi-parallel shocks to be efficiently accelerated. In the picture of DSA, particles gain energy while they are scattered of magnetic inhomogeneities back and forth across the shock front. Hence, one of the keys for efficient DSA are the magnetic inhomogeneities in the shock upstream and downstream. However, only at quasi-parallel shocks, cosmic-ray protons are able to induce magneto-hydrodynamical instabilities that again cause such inhomogeneities to grow. At quasi-perpendicular shocks, the growth of such instabilities  is prevented for two reasons \citep[also see the discussion in][]{2014ApJ...783...91C}
citep{2016Galax...4...71W,2017MNRAS.464.4448W,Roh2019,Banfi2020}. These works showed that, to first order, the distribution of shock obliquities in the ICM follows the distribution of angles between two random vectors in a three dimensional space, that is $\propto \sin \left( \theta \right)$, see top panel in Fig. \ref{fig::obli}. Hence, only $\sim 33 \ \%$ of all shocks are expected to be quasi-parallel. Additionally, the excess of quasi-perpendicular shocks over quasi-parallel shocks is somewhat larger than for a pure random distribution, as shock waves amplify the perpendicular component of the magnetic field leading to more quasi-perpendicular shocks \citep{2017MNRAS.464.4448W}. Using a larger set of cosmological simulations, \cite{Banfi2020} measured the obliquity distribution in clusters, filaments and voids. They found that locally this excess can be up to factors of $\sim 5$ larger than for the random case. Furthermore, the  excess of quasi-perpendicular shocks is maximized for Mach numbers with $5 \le M \le 20$ \citep[also see][]{2016Galax...4...71W} but it typically depends on the pre-shock temperature. Furthermore, the excess is maximized around filaments, where the shock is perpendicular to the filaments, see Fig. \ref{fig::obli}. Here, the magnetic field aligns with the filaments because of an equilibrium process that aligns local magnetic field with the density gradient as found by \cite{soler2017}
citep{2016Galax...4...71W,2017MNRAS.464.4448W,wittor2020gammas}. It is worth to notice, that the obliquity requirement does not affect the emission from radio relics. In a complementary work, \cite{Guo_eta_al_2014_I} found that cosmic-ray electrons are only efficiently accelerated by quasi-perpendicular shocks. Therefore, most shocks in the ICM, i.e. $\sim 66 \ \%$, are able to accelerate cosmic-ray electrons which leaves the power of relics almost unaltered \citep{2016Galax...4...71W,2017MNRAS.464.4448W}
cite{2017MNRAS.464.4448W} and \cite{Banfi2020}. Top left: pre-(blue) and post-shock (red) obliquity distribution of the relic simulated in \cite{2017MNRAS.464.4448W} compared to the distribution of angles for a random distribution. Top right: obliquity distribution measured for different magnetic field seeding models \citep[colored lines, see][for details]{Banfi2020} compared to the distribution of angles between two random vectors in a three dimensional space (black dotted lines). Bottom panel: spacial distribution of obliquities in two galaxy clusters. The gray color gives the ICM density. The blue squares mark quasi-perpendicular shocks, while the red squares highlight quasi-parallel shocks.}
cite{Ha2018protons} studied on the proton acceleration by low Mach number shocks in high $\beta$ plasmas. They showed that under such conditions only supercritical shocks are able to accelerate cosmic-ray protons, i.e. the acceleration is quenched for shock with Mach numbers below $M \lesssim 2.25$. Most shocks in the ICM are weak \citep{ryu2003,Vazza:2009_shock,2013ApJ...765...21S,Ha2018mergershocks,wittor2019pol} and, hence, the supercritical-requirement reduces the number of shocks, that are able to accelerate protons, significantly. However, \cite{wittor2020gammas}
cite{Ha2019gammas} tested if shock accelerated cosmic-ray protons become invisible to the Fermi-LAT if: a) the shock efficiencies are the ones derived by \cite{Ryu2019}, and b) only supercritical and quasi-parallel shocks are able to accelerated cosmic-ray protons. Using a particle-mesh/Eulerian cosmological hydrodynamic \citep{ryu1993}, they simulated 58 galaxy clusters that cover a mass range of $10^{14}-5\cdot 10^{14} \ \Msun$. In their simulation, they evolved the magnetic fields passively using the Biermann Battery mechanism \citep{Biermann}. As they did not self-consistently follow the transport of cosmic-ray protons, they computed the $\gamma$-ray emission in post-processing. Therefore, they identified all shocks in their simulation at redshift $z = 0$ and measured their properties such as strength, obliquity and energy flux. By assuming a radial distribution of cosmic-ray protons, they computed the volume-integrated momentum distribution of cosmic-ray protons that is produced by the detected shocks. Finally, they estimated the associated $\gamma$-ray emission by applying the formalisms of \cite{pe04,kelner2006}. They find that only $\sim 7 \ \%$ of the kinetic energy flux is processed by supercritical and quasi-parallel shocks. In addition, the shocks that are able to accelerate cosmic-ray protons have an average strength of $M \approx 2.8 - 3.3$. The $\gamma$-ray emission in the simulation was compared to the upper limits of the cluster sample given in \cite{ackermann14}, see Fig. \ref{fig::ha2019}
cite{Ha2019gammas}: The various panels compare the $\gamma$-ray luminosities, as a function of cluster mass, of the simulated sample (black dots) with the upper limits produces by the Fermi-LAT \citep[red crosses][]{ackermann14}. The luminosities have been computed/measured in the energy band $[0.5,200] \ \GeV$. The different panels give the results for different spatial distributions of the cosmic-ray protons, i.e. $n_{\mathrm{CR}}(r) \propto n_{\mathrm{gas}}(r)^{\delta}$. The first three panels, (a)-(c), show the luminosities with re-acceleration included, while in the last panel, (d), re-acceleration was neglected. The blues lines give the mass-luminosity relation, $L_{\gamma} \propto M_{200}^{5/3}$. }
cite{wittor2020gammas} combined cosmological simulations and La\-grang\-ian tracer particles to study the cosmic-ray proton acceleration in four massive galaxy clusters, i.e. $5.4 \cdot 10^{14}- 1.1 \cdot 10^{15} \ \Msun$ (see Fig. \ref{fig::maps}). In their modelling, they applied the acceleration efficiencies derived by \cite{Ryu2019}. In addition, they measured the reduction of the $\gamma$-ray flux if a) only supercritical shocks, b) only quasi-parallel shocks and c) only both supercritical and quasi-parallel shocks are able to accelerate cosmic-ray protons. In agreement with the results of \cite{Ha2019gammas}, they found that, using the acceleration efficiencies from \cite{Ryu2019}, the associated $\gamma$-ray emissions is invisible to the Fermi-LAT, if only supercritical and quasi-parallel shocks are able to accelerate cosmic-ray protons, see Fig. \ref{fig::gamma_vs_limits_all_cluster}
cite{wittor2020gammas}: The plot compares the total $\gamma$-ray flux the simulated sample of \cite{wittor2020gammas} with the upper limits given by the Fermi-LAT. Specifically, the grey crosses give the limites in the energy range $[0.5,200] \ \GeV$ \cite{ackermann14}. The red solid cross marks the deeper upper limit of the COMA cluster \cite{ackermann16}, while the red dashed cross is the expected upper limit after ten more years of Fermi-LAT observations of COMA. The different colored symbols give the $\gamma$-ray fluxes computed for the simulated sample. The model that combines the acceleration efficiencies from \cite{Ryu2019} with acceleration by supercritical and quasi-parallel shocks only is given by the red squares. The other models are: all shocks (black asterisks), only supercritical shocks (blue diamonds) or only quasi-parallel shocks (green triangles) are able to accelerate cosmic-ray protons. The black crosses display the $\gamma$-ray flux obtained for the ``old'' acceleration efficiencies calculated by \cite{2013ApJ...764...95K}. (The plot has been modified from its original version to fit the style of this paper).}
citep[e.g.][]{2013ApJ...764...95K} and, hence, they can inject a larger fraction of cosmic-rays. Furthermore, it is still uncertain whether re-acceleration works at every type of shock or if it is restricted to supercritical \citep{Ha2018protons} and quasi-parallel \citep{2014ApJ...783...91C}
cite{Ha2019gammas} also tested their model for cosmic-ray re-acceleration. In their model, cosmic-protons are shock accelerated at three fixed periods. While the first acceleration event is pure thermal acceleration, the second and third event also include re-acceleration. Their estimation yields that about $\sim 6 - 8 \ \%$ of pre-existing cosmic-ray protons undergo re-acceleration. Assuming that only quasi-parallel and supercritical shocks are able to re-accelerate cosmic-ray protons, they found that the energy stored in cosmic-ray protons increases about $\sim 60 \ \%$ on average. Yet, the associated $\gamma$-ray emission still remains below the Fermi-limits, see Fig. \ref{fig::ha2019}
cite{2011A&A...527A..99E} were the first to propose that cosmic-ray protons could stream out of the central regions and, hence, flattening the cosmic-ray protons profiles. Though, it is difficult to explain the lack of $\gamma$-ray emission in galaxy clusters that host radio halos with cosmic-ray streaming \citep[e.g.][and references therein]{vanweeren2019review}. However, cosmic-ray streaming is complex topic as it depends on the interactions between cosmic-rays and plasma waves and turbulence. Hence, we point the interested reader to sophisticated works and the references therein: \cite{2017MNRAS.465.4800P,2011A&A...527A..99E,2013MNRAS.434.2209W,2014MNRAS.438..124Z,2018MNRAS.473.3095W}
citep[e.g.][]{Murase2008,Murase2013,MuraseWaxman2016,Zandanel2015}. However, these works also showed that shock accelerated cosmic-ray protons do not produce significant fraction of the neutrino flux measured by IceCube\footnote{https://icecube.wisc.edu/}. Nevertheless, \cite{Ha2019gammas} computed the neutrino flux in their sample of simulated galaxy clusters (see Sec. \ref{sec::shocksandprotons}). They estimated that the neutrino fluxes in their sample are significantly below both the atmospheric neutrino fluxes at $E \le 1 \ \mathrm{TeV}$ and the IceCube flux at $E = 1 \ \mathrm{PeV}$ \cite[][respectively]{Richard2016,Aartsen2014}. Hence, they concluded that the detection of neutrinos, coming from the collisions of cosmic-ray protons and protons, is more than unlikely with the current and future generation of ground based neutrino telescopes, i.e. IceCube \citep{IceCubeRevPaper2010}, Super-Kamiokande \citep{2019ApJ...887L...6H} or future Hyper-Kamiokande \citep{2011arXiv1109.3262A}
citep{Ryu2019}, then they efficiencies become significantly smaller than previously estimated. If these new efficiencies are paired with the fact that only supercritical \citep{Ha2018protons} and quasi-parallel \citep{2014ApJ...783...91C} shocks are able accelerated cosmic-ray protons, then the expected $\gamma$-ray signal from the ICM drops below the upper limits given by the Fermi-LAT \citep{Ha2019gammas,wittor2020gammas}
cite{wittor2020gammas} showed that, even after ten more years of operation, the Fermi-LAT will most-likely not detect such a signal, see Fig. \ref{fig::gamma_vs_limits_all_cluster}
citep{CTA}
citep[AMEGO][]{amego}

